DRIBO: Robust Deep Reinforcement Learning via Multi-View Information Bottleneck

Deep reinforcement learning (DRL) agents are often sensitive to visual changes that were unseen in their training environments. To address this problem, we leverage the sequential nature of RL to learn robust representations that encode only task-relevant information from observations based on the unsupervised multi-view setting. Specifically, we introduce a novel contrastive version of the Multi-View Information Bottleneck (MIB) objective for temporal data. We train RL agents from pixels with this auxiliary objective to learn robust representations that can compress away task-irrelevant information and are predictive of task-relevant dynamics. This approach enables us to train high-performance policies that are robust to visual distractions and can generalize well to unseen environments. We demonstrate that our approach can achieve SOTA performance on a diverse set of visual control tasks in the DeepMind Control Suite when the background is replaced with natural videos. In addition, we show that our approach outperforms well-established baselines for generalization to unseen environments on the Procgen benchmark. Our code is open-sourced and available at https://github. com/BU-DEPEND-Lab/DRIBO.

==> Makefile <==
.DEFAULT_GOAL := default

# default goal
default: pdf clean

## Create PDF
pdf:
#	latex paper.tex
#	bibtex paper.aux
#	latex paper.tex
#	latex paper.tex
#	dvips paper.dvi -o paper.ps -t letter -Ppdf -G0
#	ps2pdf paper.ps
	pdflatex paper.tex
	bibtex paper.aux
	pdflatex paper.tex
	pdflatex paper.tex
	pdflatex paper.tex

## Cleanup build files
clean:
	rm -rf paper.log paper.out paper.aux paper.blg paper.bbl paper.bcf paper.run.xml paper.dvi paper.ps

## Show this help screen
help:
	@printf "Available targets\n\n"
	@awk '/^[a-zA-Z\-\_0-9]+:/ { \
		helpMessage = match(lastLine, /^## (.*)/); \
		if (helpMessage) { \
		helpCommand = substr($$1, 0, index($$1, ":")-1); \
		helpMessage = substr(lastLine, RSTART + 3, RLENGTH); \
		printf "%-30s %s\n", helpCommand, helpMessage; \
		} \
		} \
		{ lastLine = $$0 }' $(MAKEFILE_LIST)

